How to Understand Named Entities: Using Common Sense for News Captioning

News captioning aims to describe an image with its news article body as input. It greatly relies on a set of detected named entities, including real-world people, organizations, and places. This paper exploits commonsense knowledge to understand named entities for news captioning. By ``understand'', we mean correlating the news content with common sense in the wild, which helps an agent to 1) distinguish semantically similar named entities and 2) describe named entities using words outside of training corpora. Our approach consists of three modules: (a) Filter Module aims to clarify the common sense concerning a named entity from two aspects: what does it mean? and what is it related to?, which divide the common sense into explanatory knowledge and relevant knowledge, respectively. (b) Distinguish Module aggregates explanatory knowledge from node-degree, dependency, and distinguish three aspects to distinguish semantically similar named entities. (c) Enrich Module attaches relevant knowledge to named entities to enrich the entity description by commonsense information (e.g., identity and social position). Finally, the probability distributions from both modules are integrated to generate the news captions. Extensive experiments on two challenging datasets (i.e., GoodNews and NYTimes) demonstrate the superiority of our method. Ablation studies and visualization further validate its effectiveness in understanding named entities.

==> sec_bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/People/Yanhui_Wang.jpg}}]{Yanhui Wang} received the bachelor’s  degree from Tianjin University. He is currently pursuing the Ph.D.degree with the School of Electronic and Information Engineering, Tianjin University, Tianjin, China.
His research interests include but not limited to multimedia content analysis and understanding, computer vision and machine learning.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/People/Ning_Xu.jpg}}]{Ning Xu}
received the Ph.D. degree in electronic engineering from Tianjin University, China, in 2019.

He is currently an assistant professor with the School of Electrical and Information Engineering, Tianjin University.
He was a visiting scholar with the SeSaMe Centre of National University of Singapore from 2016 to 2017.
His current research interests include computer vision and machine learning.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/People/An-An_Liu.jpg}}]{An-An Liu}
(M'10) received the Ph.D. degree in electronic engineering from Tianjin University, China.

He is currently a Professor with the School of Electrical and Information Engineering, Tianjin University. He was a Visiting Professor with the SeSaMe Centre of National University of Singapore, and a Visiting Scholar with the Robotics Institute, Carnegie Mellon University, Pittsburgh, PA, USA. His current research interests include computer vision and machine learning.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/People/Yongdong_Zhang.jpg}}]{Yongdong Zhang}  %
(M'08-SM'13) received the Ph.D. degree in electronic engineering from Tianjin University, Tianjin, China, in 2002. He is currently a Professor with the School of Information Science and Technology, University of Science and Technology of China. His current research interests are in the fields of multimedia content analysis and understanding, multimedia content security, video encoding and streaming media technology.

He has authored over 100 refereed journal and conference papers. He was a recipient of the Best Paper Awards in PCM 2013, ICIMCS 2013, and ICME 2010, the Best Paper Candidate in ICME 2011. He serves as an Editorial Board Member of \emph{Multimedia Systems} Journal and the IEEE TRANSACTIONS ON MULTIMEDIA.
\end{IEEEbiography}
